Fine-Grained Scheduling for Containerized HPC Workloads in Kubernetes Clusters

Containerization technology offers lightweight OS-level virtualization, and enables portability, reproducibility, and flexibility by packing applications with low performance overhead and low effort to maintain and scale them. Moreover, container orchestrators (e.g., Kubernetes) are widely used in the Cloud to manage large clusters running many containerized applications. However, scheduling policies that consider the performance nuances of containerized High Performance Computing (HPC) workloads have not been well-explored yet. This paper conducts fine-grained scheduling policies for containerized HPC workloads in Kubernetes clusters, focusing especially on partitioning each job into a suitable multi-container deployment according to the application profile. We implement our scheduling schemes on different layers of management (application and infrastructure), so that each component has its own focus and algorithms but still collaborates with others. Our results show that our fine-grained scheduling policies outperform baseline and baseline with CPU/memory affinity enabled policies, reducing the overall response time by 35% and 19%, respectively, and also improving the makespan by 34% and 11%, respectively. They also provide better usability and flexibility to specify HPC workloads than other comparable HPC Cloud frameworks, while providing better scheduling efficiency thanks to their multi-layered approach.

==> 6.relatedwork.tex <==
\section{Related Work}\label{sec:relatedwork}

Former works in this area have focused on deploying containerized HPC workloads in traditional HPC systems. These systems have batch-oriented workload managers or resource managers, such as Slurm \cite{slurm} or Torque, and some of them have included container support \cite{slurmcontainer}. The convergence between HPC systems and Cloud environments has been also explored \cite{Zhou2021}\cite{dividenodes}, but these works mainly divide the nodes into clusters for different usage and enable the access to the HPC cluster from the Cloud cluster. 

Once the HPC workloads are containerized, they could run on Cloud environments by directly using container orchestration platforms, such as Kubernetes, Docker Swarm, and Mesos.
Beltre et al. \cite{Data2019}\cite{pankaj2018} did some performance analysis on enabling HPC workloads on Cloud infrastructure. They analyzed the HPC workload performance while using different container orchestrators like Kubernetes and Docker Swarm and different networks like InfiniBand. They used the Kubernetes default scheduler. 
Misale et al. \cite{kubeflux} introduced KubeFlux, a Kubernetes plugin scheduler that is based on Flux graph-based scheduler. This plugin translates the Pod into a Flux job and uses the policy within Fluxion to allocate jobs.
Saha et al. \cite{Saha2019} showed how MPI applications can be scheduled by Mesos using a policy-based approach. 

There are also some works focusing on the policies for scheduling HPC jobs in the Cloud. For instance,
Gupta et al.\cite{hpccloud2016} presented novel heuristics for online application-aware job scheduling in multi-platform environments.
Fu et al. \cite{yuqi2019} proposed a progress-based container placement for short-lived containerized jobs. 
Aupy et al.\cite{researve2019} provided an optimal job reservation strategy in scheduling to minimize the cost.

Kubernetes ecosystem community is definitely an important contributor in this area. For instance, Kubeflow MPI operator \cite{kubeflowmpi} provides a better specification for MPI applications and Volcano \cite{volcanompi} features batch scheduling capability that Kubernetes lacks by providing some policies/plugins to enable optimized scheduling for jobs. Details of Kubeflow and Volcano have been discussed in Section \ref{sec:background}.

HPC community has important performance considerations on its workloads. Therefore, trialing new deployment schemes for different types of HPC workloads to improve their performance is necessary. Walkup et al. \cite{bestpractice2022} reported best practices for running compute-, memory-, and network-intensive HPC workloads on the Cloud. Medel et al. \cite{MEDEL2018286} conducted a performance analysis over Kubernetes considering the deployment and initialization overhead as well as understanding the performance of different Pod settings. Moreover, they provided a rule to decide the number of containers per pod by considering the characteristics of the application. 
% Our previous 
Our previous papers\cite{Liu2020}\cite{Liu2021} demonstrated systematically that i) some types of containerized HPC applications can exploit multi-container deployments which partition the processes that belong to each application into multiple containers in each host in order to achieve better performance; ii) some types of HPC applications gain benefits when using containers by constraining them to a single NUMA domain or pinning to specific processors. These works show some ways in the Cloud to achieve better performance for HPC workloads, but those insights are not yet being integrated and utilized by the current Cloud schedulers.





